Exploring the properties of low-frequency radio emission and magnetic fields in a sample of compact galaxy groups using the LOFAR Two-Metre Sky Survey (LoTSS)

We use the LOFAR Two-metre Sky Survey (LoTSS) Data Release I to identify the groups of galaxies (and individual galaxies) from the Hickson Compact Groups and Magnitude Limited Compact Groups samples that emit at the frequency of 150\,MHz, characterise their radio emission (extended or limited to the galaxies), and compare new results to earlier observations and theoretical predictions. The detection of 73 systems (and 7 more -- probably) out of 120, of which as many as 17 show the presence of extended radio structures, confirms the previous hypothesis of the common character of the magnetic field inside galaxy groups and its detectability. In order to investigate the future potential of low-frequency radio studies of galaxy groups, we also present a more detailed insight into four radio-emitting systems, for which the strength of the magnetic field inside their intergalactic medium (IGM) is calculated. The estimated values are comparable to that found inside star-forming galaxies, suggesting a dynamical and evolutionary importance of the magnetic field in galaxy groups.

==> old_table.tex <==
%====================================
\begin{table*}[ht]
\caption{\label{tab:fluxes}Basic data on the sample systems, as well as total flux density (in mJy) measured in LoTSS, FIRST, and NVSS. All data are from \citealt{mlcg}, unless stated otherwise.}
\begin{center}
\begin{tabular}{lccccccccc}
\hline
\hline
System		& $\rm N_G$	&		 z					&		D		&	$\sigma_{V}$		&		$\Phi$	&	LoTSS-6			&	LoTTS-20		&	FIRST			&	NVSS		\\
  &  &  & [kpc][{\bf Mpc?}] & [km/s] & [kpc] & [mJy] & [mJy] & [mJy] & [mJy] \\
\hline
HCG 60		&	3		&	0.0625 $\pm$  0.0005	&	255 $\pm$ 2		&	421 $\pm$ 72			&		38.6 $\pm$ 4	&	2409 $\pm$ 91	&	2444 $\pm$ 122	&	324 $\pm$ 14	&	655 $\pm$ 33	\\
MLCG 24		&	3		&	0.0691 $\pm$  0.0006	&	282 $\pm$ 2		&	353 $\pm$ 60			&		22 $\pm$ 4.6	&	926 $\pm$ 46	&	934 $\pm$ 47	&	180 $\pm$ 9		&	223 $\pm$ 11	\\
MLCG 41		&	4		&	0.0154 $\pm$  0.0000	&	63 $\pm$ 1	*	&	33	$\pm$ 6				&		36.8 $\pm$ 4	&	15 $\pm$ 1	&	14.3 $\pm$ 0.7	&	3.1**$\pm$ 0.2	&	4.7 $\pm$ 0.5	\\
MLCG 1374	&	3		&	0.0697 $\pm$  0.0003	&	285 $\pm$ 2		&	177 $\pm$ 36			&		95.6 $\pm$ 15.8	&	27 $\pm$ 1	&	26.6 $\pm$ 1.3	&	4.8 $\pm$ 0.3	&	5.5 $\pm$ 0.5	\\

\hline
\end{tabular}
\end{center}
Description of columns:\\
$\rm N_{G}$ -- number of galaxies in the group;\\
z -- redshift {\bf [photometric? spectroscopic?]};\\
D -- distance to the system, calculated from redshift, assuming $\rm H_0$ = 73 km/s/Mpc, in [kpc] {\bf [wouldn't be Mpc]};\\
$\sigma_{V}$ -- velocity dispersion, in [km/s];\\
$\Phi$ -- physical diameter of the system (from optical data), in [kpc];\\
The last four columns contain the flux densities from the respective survey data, in [mJy].\\
* reported z uncertainty was 0, therefore 1\,Mpc uncertainty for distance estimate was assumed\\
** signal-to-noise ratio does not exceed 2.8.\\
\end{table*}
%====================================
